MotionDeltaCNN: Sparse CNN Inference of Frame Differences in Moving Camera Videos

Convolutional neural network inference on video input is computationally expensive and requires high memory bandwidth. Recently, DeltaCNN managed to reduce the cost by only processing pixels with significant updates over the previous frame. However, DeltaCNN relies on static camera input. Moving cameras add new challenges in how to fuse newly unveiled image regions with already processed regions efficiently to minimize the update rate - without increasing memory overhead and without knowing the camera extrinsics of future frames. In this work, we propose MotionDeltaCNN, a sparse CNN inference framework that supports moving cameras. We introduce spherical buffers and padded convolutions to enable seamless fusion of newly unveiled regions and previously processed regions -- without increasing memory footprint. Our evaluation shows that we outperform DeltaCNN by up to 90% for moving camera videos.

==> figures/padding/padding_figure.tex <==
\begin{figure*}[pt]
\begin{subfigure}{.04\linewidth}
a
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frame1.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/out1_original.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frame2.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/correct_f2.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frames_fused.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/correct_fused.png}
\end{subfigure}


\begin{subfigure}{.04\linewidth}
b
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frame1.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/out1_original.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/delta2.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/out2_original.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frames_fused.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/accumulated_original.png}
\end{subfigure}%

\begin{subfigure}{.04\linewidth}
c
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frame1.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/out1_dilated.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/delta2.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/out2_dilated.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/frames_fused.png}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \includegraphics[width=.95\linewidth,valign=c]{figures/padding/accumulated_dilated.png}
\end{subfigure}%

\begin{subfigure}{.04\linewidth}
  \centering
  \caption*{}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Input 1}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Output 1}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Input 2}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Output 2}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Fused in.}
\end{subfigure}%
\begin{subfigure}{.155\linewidth}
  \centering
  \caption*{Fused out.}
\end{subfigure}%

\caption{
Padded convolutions (c) enable buffer growth over previously unseen regions without artifacts.
In this example, we apply a 3x3 average filter on the input.
Row a: standard convolution without padding - only the 3x3 pixels containing actual values are processed. The fused output is generated by processing all 4x3 pixels at once.
Row b: \ours without padding - only the Delta of the current 3x3 pixels is processed - newly unveiled pixels lack knowledge of their neighboring pixels' accumulated values. The fused output does not match that of row \emph{a} in the newly added column.
Row c: \ours with padding - by processing all pixels that are affected by the current input, newly unveiled pixels include all accumulated values of their neighbors. The fused output of row \emph{c} matches that of row \emph{a} for the newly added column.
% \markus{which images should fully match now?}
}
\label{fig:dilated_padded_convolution}
\end{figure*}
